Understanding Data Science Lifecycle Provenance via Graph Segmentation and Summarization

Increasingly modern data science platforms today have non-intrusive and extensible provenance ingestion mechanisms to collect rich provenance and context information, handle modifications to the same file using distinguishable versions, and use graph data models (e.g., property graphs) and query languages (e.g., Cypher) to represent and manipulate the stored provenance/context information. Due to the schema-later nature of the metadata, multiple versions of the same files, and unfamiliar artifacts introduced by team members, the "provenance graph" is verbose and evolving, and hard to understand; using standard graph query model, it is difficult to compose queries and utilize this valuable information. In this paper, we propose two high-level graph query operators to address the verboseness and evolving nature of such provenance graphs. First, we introduce a graph segmentation operator, which queries the retrospective provenance between a set of source vertices and a set of destination vertices via flexible boundary criteria to help users get insight about the derivation relationships among those vertices. We show the semantics of such a query in terms of a context-free grammar, and develop efficient algorithms that run orders of magnitude faster than state-of-the-art. Second, we propose a graph summarization operator that combines similar segments together to query prospective provenance of the underlying project. The operator allows tuning the summary by ignoring vertex details and characterizing local structures, and ensures the provenance meaning using path constraints. We show the optimal summary problem is PSPACE-complete and develop effective approximation algorithms. The operators are implemented on top of a property graph backend. We evaluate our query methods extensively and show the effectiveness and efficiency of the proposed methods.

==> system_overview.tex <==
%!TEX root = main_sigmod.tex
\section{System Implementation}
\label{sec:system}

The proposed techniques are implemented in our provenance management system (\provdb)~\cite{provdb@hilda17}, shown in
Fig.~\ref{fig:sys_arch}, with the two operators that are the focus of this paper highlighted. %Our focus in this work are the proposed \prov\ provenance graph operators which are highlighted in the figure. 
%
When used by data science team in practice, \provdb\ is designed to work behind the scenes in a nonintrusive manner. It collects
provenance via a \cmd{git}-like command line interface (CLI) called \cmd{provdb}, which is prefixed over command line executions of
day-to-day commands (e.g., \cmd{provdb cp model.config new\_model.config}) by the users.  The context of the executed command (Activity,
        User) and changes of project artifacts (Entity) occurred before/during/after the execution are captured by \cmd{provdb} and
stored in a property graph store. \provdb\ can also act as a data version control system (DVCS) for data science project artifacts like
large model files consisting of float numbers~\cite{modelhub@icde17}, for which \cmd{git} performs poorly~\cite{dvcs@vldb15}.
    
    %to
%manage the versioned project artifacts. It is tailored for analytics project artifacts like large model files mainly consisting of float numbers. 
%It features with new versioning algorithms~\cite{modelhub@icde17} for such artifacts instead of simple \cmd{git} heuristics which often performs poorly other than plain files~\cite{dvcs@vldb15}. 

Once versions of the project artifacts and provenance of the team activities are managed by \provdb, the data science team members and stakeholders are able to analyze the lifecycle provenance. 
To better utilize lifecycle provenance, \provdb\ provides a rich set of specialized query facilities assembled in a HTML frontend, and
also allows using Cypher to query the provenance graph directly. 
The segmentation and summarization operators proposed in this paper are implemented with templated query interface in the front end: 
\textbf{a)} for \opseg, the users identify snapshots of interest via search interface and specify boundary criteria within HTML GUI; 
\textbf{b)} for \opsum, previous \opseg\ results are selectable in the GUI and the property aggregation and the provenance type can be specified accordingly. 
Returned results of both operators can be visualized and interacted with via \cmd{d3.js}. \lowPriority{Beyond the query operators discussed in this paper, \provdb\ supports several template queries, such as exploring the version artifacts, managing pipelines, and monitoring particular property values. }More details about other features and query types of interest are described in~\cite{provdb@hilda17}.
%
The query execution engine for the proposed operators and their algorithms\sigmodeat{ (Sec.~\ref{sec:query})} are implemented in Java using Neo4j in embedded mode for better performance. 

\lowPriority{
%\outline{other issues we avoid to address and our rationale}
\topic{Discussion:} Note the design decision of using a general purpose native graph backend (Neo4j) for high-performance provenance ingestion may not be ideal, as the volume of ingested provenance records would be very large in some applications, e.g., whole-system provenance recording at kernel level~\cite{pass_harvard@atc06,linuxprov_abates@atc15} would generate GBs of data in minutes. The support of flexible and high performance graph ingestion on modern graph databases and efficient query evaluation remain an open question~\cite{dda_microsoft@cidr17}. We leave the issue to support similar operators for general \prov\ graph for our future steps. The proposed techniques in the paper focus on enabling better utilization of the ingested provenance information via novel query facilities and are orthogonal to storage layers in provenance systems. 
}

